Towards Automatic Parsing of Structured Visual Content through the Use of Synthetic Data

Structured Visual Content (SVC) such as graphs, flow charts, or the like are used by authors to illustrate various concepts. While such depictions allow the average reader to better understand the contents, images containing SVCs are typically not machine-readable. This, in turn, not only hinders automated knowledge aggregation, but also the perception of displayed in-formation for visually impaired people. In this work, we propose a synthetic dataset, containing SVCs in the form of images as well as ground truths. We show the usage of this dataset by an application that automatically extracts a graph representation from an SVC image. This is done by training a model via common supervised learning methods. As there currently exist no large-scale public datasets for the detailed analysis of SVC, we propose the Synthetic SVC (SSVC) dataset comprising 12,000 images with respective bounding box annotations and detailed graph representations. Our dataset enables the development of strong models for the interpretation of SVCs while skipping the time-consuming dense data annotation. We evaluate our model on both synthetic and manually annotated data and show the transferability of synthetic to real via various metrics, given the presented application. Here, we evaluate that this proof of concept is possible to some extend and lay down a solid baseline for this task. We discuss the limitations of our approach for further improvements. Our utilized metrics can be used as a tool for future comparisons in this domain. To enable further research on this task, the dataset is publicly available at https://bit.ly/3jN1pJJ

==> IEEEconf_ICPR2020/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> IEEEconf_ICPR2020/rebuttal/rebuttal.tex <==


% \documentclass[10pt,twocolumn]{article}
% \begin{document}




\section{Rebuttal}
We would like to thank all the reviewers for their thoughts and valuable feedback on our work of automatically recovering graph structures from SVC. We incorporate these into the revised version of our work.
We are glad that the reviewers agree on the relevance of our proposed dataset, which enables machine learning techniques to conquer the problem of automatic analysis of SVC. As a result to the comments of Reviewers \#3 and \#5 we decided to make the dataset available at \href{https://bit.ly/3jN1pJJ}{https://bit.ly/3jN1pJJ} prior to publication. We also show additional results in the supplementary. We further address some common concerns of the reviewers below:

\textcolor{red}{\textbf{Reviewer \#3}}:
\textbf{``A simplification of the adopted metrics should be considered [\dots]"}:
We understand that as the metrics are not widespread they are more difficult to interpret. However, applying a simplified variant to display errors graph reconstruction seems difficult. While one could consider the cardinality of missing node/edge sets this metric would struggle with not being normalised and thus has very little meaningfulness. We display the normalised values in our evaluation scheme for the individual detection of nodes and edges also in Table 2.

\textcolor{red}{\textbf{Reviewer \#4}}:
% \textbf{How does angled edges been recognized in our representation and in the dataset?}
\textbf{On the representation of angled edges}:
% We have chosen the corners of the bounding box of an angled edge as the start and end point of the arrow. For an example, we have thus classified an angled edge that starts in the upper left corner and goes across the upper right corner to the lower right corner as tl2br and resprectiv to this as an diagonal edge. Therefore, our goal was to identify every type of edges in a uniform way as a whole and not as two edges. 
% Alternative: 
We define edge types by their start and end point within their bounding box.  Therefore, an angled edge with a corner and a diagonal edge have the same class label, if they both start and end in the same corners. The exact path, whether its straight for a diagonal edge or angled for an edge with one corner, is irrelevant in this implementation.
Even future work with rounded edges could be implemented in this way.
Our reasoning behind this decision was that for the graph reconstruction we are typically not interested in the type of path an edge takes as their drawings can become quite convoluted, and, thus, only focus on the general connection between nodes.

As such the angled edges are not overlooked, but they face similar problems as not angled edges with the detection of the directions (specifically the detection of arrow tips). The direction of the edge is a difficult task, as the only difference between \textit{i.e.} a bidirectional arrow and an unidirectional one is the head of the arrow. This is a common reason for errors on the synthetic and on the real-world dataset. We have clarified these concerns in the main paper.

\noindent\textbf{``Table 1 is a little confusing, because of mixing \#labels and mAP without explicitly labelling the rows in the table."}:
We acknowledge this and we have clarified Table 1 in the revised version. 
Furthermore, we appreciate Reviewer \#4's stance on our evaluation. Since there are, to the best of our knowledge, no results that address exactly the recognition of structure and the building of representations within flow charts, straight comparisons were not possible. On a related note, we see this as additional aspect of our work to shed light on this problem to enable comparison and mutual improvement for the analysis of SVC.


\textcolor{red}{\textbf{Reviewer \#5}}:
\textbf{``The idea to generate synthetic data for such kind of
problem is not new [\dots]"}:
While the use of synthetic data has been increasing recently for various vision domains including document analysis, there currently exists no work which allows for the concrete analysis of structured visual content the same way as our SSVC.
Even though the core idea of our dataset generation approach can be easily extended in many ways, we show
% The main contribution lies in the presented set of minimal requirements a dataset for this task has to have and we show that 
this iteration of our dataset already enables machine learning models to handle several problems of SVC well. This does not only include the SVC images themselves, but also all the ground truth information for the object detection and the graph representation.

The size of the generated dataset is not limited in any way and the richness of content in the SVCs can be extended and adapted to the desired needs. 
% While we publish this dataset, it should be noted that this is not a final and perfect dataset. 
We note, that this is a base that can be used for comparison and future work can construct larger more complex versions following our proposed pattern.

\noindent\textbf{``[\dots]~the dataset suffers from unrealistic representations."}:
It has to be said that the data set certainly contains representations that are not realistic in terms of a perfect and beautiful flow chart. But most of them are comparable to examples in the DISKNET dataset. Here, many of the graphs created by humans are not unambiguous and present the same "unrealistic" representations. Similarly, the appearance of text seems to be sometimes better and sometimes worse, especially in relation to the placement of legends. 
Our experiments showed that a machine learning model trained on our dataset is able to learn the core concepts and can handle more difficult data in the training than it may see in the real application later. Therefore, it is no problem to include difficult and rarely unrealistic representations if the core concept is similar enough to the desired application.
% The aim here was to make the representations more difficult to learn a more difficult problem rather than an easier problem, as this would simply allow the recogniser to learn more difficult cases.


\noindent\textbf{Changes in the related work section and strengthening of the links to other works}:
We have expanded our related work in the revised version, including other graph structure generating methodologies from the field of mathematical form recognition as well as the other recommended literature. Especially the two papers on edit distance and subgraph detection show the possibilities of establishing such metrics and the difficulty of the problem. Work on table recognition or element localization is useful as a preliminary step to our work, in which the SVC must first be extracted from the document.
% Additionally, the localisation of elements within the flow chart is an important part of the pipeline. 
However, albeit several of these works being related they neither provide direct solutions to the problems of our task nor are easily transferable to it. As such we see not only our dataset but also our proposed graph extraction process from SVC as a novel contribution.




% \textbf{on the interpretability of our work}:
% % - establishing stronger links to other works,
% % - showing more examples of the dataset and the results
% % - commenting on the evaluation metrics in more detail
% % explain with reference to other paragraphs

% We understand that it is difficult to interpret the results without any comparisons to other works, but sadly there are none yet.

% This is another reason why this idea has to be published, so that it enables comparison and mutual improvement.
% We realise that in our attempt to give a very neutral and truthful presentation of the achieved results, we focused much more on the problems we want to fix, than presenting the actual goal that we achieved. The approach works very well for most graphs and often only fails at the same things a human fails when he is faced with the same SVC. It has a near 100\% detection rate of nodes and the edge detection is good enough so that the graph reconstruction works correctly in most cases. The most difficult task for now is the assignment of weights to their edges as this is often very ambiguous. In addition, the metrics are not perfect either. For example, if an edge from A to B is recognized as an edge from A to C, then it is counted as two errors since it is missing at B and wrongly added to C. Here, the main problem is to match detected edges with edges in the ground truth, but this is a very hard problem and out of the scope of this first approach.
% We tried to include those remarks and positive comments about the achieved goal now in this work and hope that future work introduces better metrics, that show the performance more clearly. We also included more positive examples in the supplementary.
% - Tabelle 1 ist mir absicht so aufgebaut (#Labels über mAP), damit zu erkennen ist, wie stark sich ein Fehler auswirkt (je weniger Labels, desto sträker der Einfluss) (R4)

\\
\vspace{5pt}
\noindent We thank the reviewers again for their time and truly
hope that our rebuttal will be considered in the discussions
before reaching a final decision.

% \clearpage



%synthetic dataset is not yet publicly available

%A simplification of the adopted metrics should be considered: it is hard to understand if the method works well or not because of a very huge set of numbers

% more examples of the generated dataset should be presented to the reader
% --> google drive
% --> supplementary

% the lack of explanation for angled edges, which are briefly mentioned, but all edge classes only represent one direction

% Table 1 is a little confusing, because of mixing #labels and mAP without explicitly labelling the rows in the table

% no comparison to other works, but if none of them are producing the same output representation, it is understandable that there cannot be any direct comparison
% --> eval comparison not possible

% The SOTA review is very short and are some missing
% reference. Ref [5][6] are not representative of the SOTA. I
% suggest for example the following:
% 1- T. N. Le, M. M. Luqman, A. Dutta, P. Heroux, C. Rigaud,
% C. Guerin, P. Foggia, J. Burie, J. Ogier, J. Llados, and S.
% Adam, � Ssgci: subgraph spotting in graph representations
% of comic book images, � Pattern recognition letters, 2018.

% 2- Z. Abu-Aisheh, B. Ga�zere, S. Bougleux, J. Ramel, L.
% Brun, R. Raveaux, P. H�roux, and S. Adam, � Graph edit
% distance contest 2016: results and future challenges, �
% Pattern recognition letters, vol. 100, p. 96�103, 2017. 

% 3- Have a look at the IAPR TC10 datasets page :
% https://iapr-tc10.univ-lr.fr/?page_id=71

%Some references to Mathematical expressions recognition (R5)

%The promise to make the dataset publicly available is not
%achieved yet.

% %dataset suffers from unrealistic representations. For
%  example textual placement is more randomly distributed in
% general than that of the dataset

% We get the impression of a
% non achieved goal if thinking at a general purpose
% representative dataset

% Disagree against no contribution

% \end{document}






==> IEEEconf_ICPR2020/sections/0_abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
Structured Visual Content (SVC) such as graphs, flow charts, or the like are used by authors to illustrate various concepts.  While such depictions allow the average reader to better understand the contents, images containing SVCs are typically not machine-readable. This, in turn, not only hinders automated knowledge aggregation, but also the perception of displayed information for visually impaired people. 
%In this work, we propose the automatic extraction of a graph representation of SVC by training deep learning models on synthetic data. 
In this work, we propose a synthetic dataset, containing SVCs in the form of images as well as ground truths. We show the usage of this dataset by an application that automatically extracts a graph representation from an SVC image. This is done by training a model via common supervised learning methods.
As there currently exist no large-scale public datasets for the detailed analysis of SVC, we propose the Synthetic SVC (SSVC) dataset comprising 12,000 images with respective bounding box annotations and detailed graph representations. Our dataset enables the development of strong models for the interpretation of SVCs while skipping the time-consuming dense data annotation. 

We evaluate our model on both synthetic and manually annotated data and show the transferability of synthetic to real via various metrics, given the presented application.
Here, we evaluate that this proof of concept is possible to some extend and lay down a solid baseline for this task. 
We discuss the limitations of our approach for further improvements.
Our utilized metrics can be used as a tool for future comparisons in this domain.
To enable further research on this task, the dataset is publicly available at \href{https://bit.ly/3jN1pJJ}{https://bit.ly/3jN1pJJ}.


% Structured visual content such as graphs, flow charts or similar cannot be perceived by visually impaired people and machines. To make this possible, we propose an approach that converts such structured visual content in to a machine-understandable representation. Previous work exists only for very restricted subfields of this task which make strong assumptions about the images. To circumvent these restrictions, we propose an approach using machine learning, which tries to solve the problem for real data by using a synthetic data set. We showed, that this is successful to some degree and discuss the limitations of this approach and propose improvements for future applications.
\end{abstract}



==> IEEEconf_ICPR2020/sections/1_introduction.tex <==


%%%%%%%%% BODY TEXT
\section{Introduction}

%Shows the process of the Original Image to the Graph representation. This leads to two paths on the left side concerning the Object Detection and the Graph Creation and on the right side the Text Recognition and the Text Mapping which uses information from the Object Detection.

\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-30pt}

\begin{figure}[t]
    \centering
    % \vspace{10pt}
    \includegraphics[width=0.85\linewidth]{IEEEconf_ICPR2020/figures/Ablauf_v5.pdf}
    \caption{This flow chart describes the steps we used to extract a graph representation from an SVC image. At first, structures and texts are detected independently. Later they are merged again by using their bounding boxes and thus results in a complete representation of the SVC.}

    \label{fig:intro}
\end{figure}


An image says more than a thousand words. Following this line of thought, in almost all fields of living one tries to convey complex concepts in a visual manner. As such, fields like engineering or teaching cannot be imagined without the use of structured visual content (SVC) in the form of flow charts, diagrams, or similar graphs~\cite{mcgrath2005visual}. While SVC allow an immense condensation of information, it becomes hard to make these types of information machine parsable and therefore it is difficult to automatically aggregate information and enable various downstream tasks, such as accessibility, \textit{e.g.}, for visually impaired people. Thus, it is necessary to translate SVC into a machine parsable structure such as a graph representation to enable further processing.

The analysis of documents is a long established problem in computer vision. Most work, hereby, focuses either on the identification of text~\cite{smith2007overview,shi2015endtoend} or segmentation of different content types ~\cite{nguyen2021tablesegnet,SPaSe,WiSe}. As such Haurilet~\etal~\cite{SPaSe,WiSe} utilize deep learning methods to partition lecture slides into their specific parts to enable further downstream tasks. While such work addresses the identification and contextualization of SVC, the SVC itself remains untouched and cannot be interpreted. Auer~\etal~\cite{optical_graph_recognition} try to reconstruct the graph representation of a well defined subcategory of SVC through the use of classical computer vision algorithms which can be susceptible to error when applied to unconsidered domains. 

\setlength{\abovecaptionskip}{6pt}
\setlength{\belowcaptionskip}{-10pt}
\begin{figure*}[t]\label{gen_img}
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.3\linewidth,height=0.23\linewidth]{IEEEconf_ICPR2020/figures/example_1006_cut_3.png}
    &
    \includegraphics[width=0.4\linewidth,height=0.23\linewidth]{IEEEconf_ICPR2020/figures/example_disknet2_1.png}  \\
    \footnotesize{(a) Example of our generated dataset.} & 
    \footnotesize{(b) Example from the DISKNET dataset.}
\end{tabular}
\caption{Comparison of a generated image (a) with a real one from the DISKNET dataset (b).}
\label{fig:example_synthetic_vs_disknet}
\end{figure*}

We observe underlying similarities between various types of SVC. Nodes relating to objects are typically represented by geometrical structures such as  boxes, ovals, etc. in varying forms whereas their relationships are displayed via different types of arrows. Despite building upon simple structures, highly complex graphs can become too difficult to interpret for handcrafted methods. To combat this issue, we propose the use of a synthetic dataset in which we artificially generate random visual graphs to train deep learning methods for the detection of nodes and their relationships. Our approach can be seen in Fig.~\ref{fig:intro}. We generate a large scale SVC dataset and propose a method to automatically parse their graph representation. We evaluate our method not only on our synthetic dataset but also on the real world DISKNET~\cite{Disknet} dataset, which among others contains various SVC which were automatically extracted from different real world papers summarized in an extensive knowledge base, to highlight both its strengths and weaknesses.

\iffalse
__________________________

As concepts get more and more complex it gets harder to explain them with words. Therefore, many explanations, presentations and research papers use visually structured content such as flow charts and graphs to aid understanding. While this is a great possibility to condense a lot of information, images are not comprehensible for everyone. 
% Visually impaired humans have so far no chance of gaining any additional information via graphical representations by themselves. 
Visually impaired people have so far hardly any possibilities to obtain information themselves via graphical representations.
% Instead, there is a lack of possibilities to transfer the information in a different way for example, through complete structural descriptions for blind people.
There are assistive technologies missing to transfer the information automatically into a perceptible way for them. This could be a structural descriptions of the graphical representation.
Furthermore, knowledge extraction or searches in those graphics are impossible, since machines can not comprehend visually structured content.
To solve this problems it is essential that machines could understand the visual content and transform it into a different representation. 
Due to the high variability of graph representations, it is hardly possible to create fixed rules that can recognise such graphical content and extract the information. 
An alternative approach is machine learning. The training of machine learning models requires a dataset that is as large as possible. 
Because of the high variability of graph representations the dataset should contain as many variations in representation and structure as possible. This paper presents an approach for automated generation of such a dataset. It also presents a first approach to extract information from such a graph using machine learning.

\fi






% % goal/use case: understand visually structured content such as flow charts for computers
% % => different representation possible, especially for visually impaired people
% As concepts get more and more complex it gets harder to explain them with words. Therefore, many explanations, presentations and research papers use visually structured content such as flow charts and graphs to aid understanding. While this is a great possibility to condense a lot of information, images are not comprehensible for everyone. Visually impaired humans have so far no chance of gaining any additional information via graphical representations by themselves. 
% Furthermore, knowledge extraction or searches in those are impossible, since machines can not comprehend visually structured content.
% %In this case and for many other possibilities it would be very helpful if a machine could understand the visual content and transform it into a different representation. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{example-image-a}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% This paper is going to discuss old approaches to solve this task and its problems and presents a novel way to conquer this task with the help of machine learning. In that approach we also show the benefits of synthetic to real learning to mitigate the lack of ground truth annotations.

% \blindtext[1-4]

==> IEEEconf_ICPR2020/sections/2_related_work.tex <==
% Related work about graph recognition
% A.  M.  Awal,  G.  Feng,  H.  Mouch`ere,  and  C.  Viard-Gaudin: First experiments on a new online handwritten flowchart database
% extract a  graph  like  structure  from  hand  drawn  flow  charts
% two  parts:  Recognizing  the  elements that  represent  the  graphical  components  and  extracting  the text  itself.

% Auer,  C.  Bachmaier,  F.  J.  Brandenburg,  A.  Gleißner,  and  J.  Reisl-huber: Optical graph recognition
% recognizing limited graph structures without text
% multi-step  procedure: pre-processing, segmentation, topology recognition, and post-processing
% mainly using conventional computer vision methods and pixel based operations

% G. Vasudevan, S. Dhanapanichkul, and R. Balakrishnan: Flowchartknowledge extraction on image processing
% extract   knowledge  from flow  charts  without  recognizing  an  explicit  graph  structure
% strict assumptions about the given images. use case only

% X-H. Wu, M.-C. Qu, Z.-Q. Liu, and J.-Z. Li: Research and application of code automatic generation algorithm based on structured flowchart
% generate  code  from  given  flowcharts
% strict assumptions about the given images. use case only

% Automatic image dataset generation
% mostly web crawling and labeling: 
% Marko Arsenovic, Srdjan Sladojevic, Andras Anderla, Darko Stefanovic, Bojan Lalic: Deep learning powered automated tool for generating image based datasets

% simple synthetic data: cracks in concrete/microchips - patch background with random cracks
% source ?
% talks about it: Digital reality: a model-based approach to supervised learning from synthetic data

% Synthetic Data Generation for Steel Defect Detection and Classification Using Deep Learning
% highly sophisticated image generation. ground truth generated? only type of crack but not location - not related to out task

% Synthetic data via GAN - many examples
% No structure in images. Learn similarities to given images.
% Unable to document what was created. We need that information to construct ground truth graph structure and bounding boxes

% Kinect: erster anwendungsfall synthetic image data
% J. Shotton et al.: Real-time human pose recognition in parts from single depth images

% Kishor Bhoyar: Synthetic Image Dataset
% images with random color segments for testing color image segmentation algorithms
% easy ground truth

% Andreas et al.: SHAPES
% dataset of synthetic images designed to benchmark systems for understanding of spatial and logical relations among multiple objects.
% rgb objects in a 3x3 grid with ground truths to learn complex questions about arrangements of colored shapes


\section{Related Work}
%The related work can be separated into two major streams, where the first one is concerned with techniques for document analysis in general (Sec.~\ref{subsec:document_analysis}) and the second one is focusing on the use case of graph recognition (Sec.~\ref{subsec:structured_visual_content}).

\iffalse
Existing work in document analysis focuses on two different domains: i) text recognition and ii) recognition of structures. 
%
% text about text recognition
%
Text recognition aims to identify text in images and transform them to machine understandable text representations. This is for example done in \cite{smith2007overview, shi2015endtoend} by methods of machine learning. 

%
% Text about structure analysis especially of graphs maybe going back to 
%
In addition there is also scientific research dealing  with the segmentation of structure in documents. Works like \cite{SPaSe,WiSe}, deal with the task of page segmentation of lecture slide content. This is done as a prerequisite step for the recognition task. Furthermore, there is also research dealing with the segmentation of tables \cite{nguyen2021tablesegnet}. 

In contrast to existing literature we combine  both streams. After using the segmentation task to identify structures like nodes and edges we use text recognition to deal with the content of the nodes and the edges. Together we use this to build the graph representation of the SVC.

\fi



\subsection{Document Analysis}
\label{subsec:document_analysis}
% \noindent\textbf{Document Analysis}
Recent works in the field of document analysis seem to focus on one of two different problems. On the one hand, the area of text recognition aims to identify text in images and transform it to machine understandable text representations. This is for example done in \cite{smith2007overview} and \cite{shi2015endtoend} by methods of machine learning.  More advanced versions even try to recognize handwritten mathematical formulas \cite{maths_handwritten} or printed formulas \cite{math_printed}.
% On the other hand the focus is set on the recognition of document structures, often via segmentation. Works like \cite{SPaSe} or \cite{WiSe}, deal with the task of page segmentation of lecture slide content. This is done as prerequisite step for the recognition task. Other works deal with the segmentation of tables \cite{nguyen2021tablesegnet}. 
On the other hand, the focus is set on the recognition of document structures, often via segmentation. Examples are the page segmentation of lecture slide content \cite{WiSe} or the detection and segmentation of tables \cite{nguyen2021tablesegnet}.
In contrast to existing literature, we combine both text recognition and content localization. Thus, after the identification of nodes and edges we utilize text recognition models to deal with their content. We use this to build the graph representation of the SVC.





\iffalse

Automatic construction of an image dataset is mostly done by web crawling methods and subsequent labeling \cite{Crawling}. When the labeling part is too expensive, methods are needed that generate images together with its labels.
While image creation techniques such as GANs provided promising results in recent times, they do lack this key feature. Besides the images, we also need ground truth information about the objects in the image and their relation to each other. \citeauthor{Kishor} demonstrates a simple example of this idea. He generates synthetic images with differently colored segments and easy ground truths. These images and ground truths can then be used to test any color image segmentation algorithm \cite{Kishor}. 



Similarly, \citeauthor{SHAPES} generate synthetic images of 3x3 geometric objects and construct fitting questions about the arrangements of these colored shapes. These complex questions can then be used as ground truths to benchmark systems for understanding of spatial and logical relations among multiple objects \cite{SHAPES}.

A great example, where synthetic data was successfully used to train a model is shown by the Xbox Kinect. Its sensor is able to recognize human poses in real-time which was made possible by training the model heavily on synthetic data \cite{Xbox}
\fi


\subsection{Structured Visual Content}
\label{subsec:structured_visual_content}
%% \noindent\textbf{Structured Visual Content: }
In regards to our use case, only little work has been done on the recognition of SVC in general. Existent research focuses on similar topics, where the detection of structure in visuals is important. 
The recognition of mathematical formulas from text often uses a tree based structure to capture the structure and relation of different components within the formula \cite{math_graph}.
Some work focuses on graph structures and the associated construction of metrics. Le~\etal~\cite{LE2018118} focuses on the recognition of subgraphs in graph representations of comic book images with state of the art methods and also addresses the availability of ground truth datasets. Possibilities of calculating the edit distance of graphs efficiently are considered in~\cite{ABUAISHEH201796}.
More closely related to our definition of SVC are the following related works.
Building upon the real-world dataset (DISKNET), Scharfenberger~\etal~\cite{scharfenberger2021augmented} train a model for the extraction of such SVC. They are however limited by the low number of manually labeled training data available for their context. Further, their research still lacks in detecting node text content and in detection of edges and assigning the weights and their text. 
Awal~\etal~\cite{handwritten} try to extract a graph-like structure from hand drawn flow charts. This separates the task into two parts. Recognizing the elements that represent the graphical components and extracting the text itself.
Auer~\etal~\cite{optical_graph_recognition} on the other hand do not consider text and concentrate on recognizing limited graph structures. Those consist only of fully colored circular nodes and bidirectional straight edges. Their work uses a multi-step procedure with pre-processing, segmentation, topology recognition, and post-processing, while mainly using conventional computer vision methods and pixel based operations. 
Vasudevan~\etal~\cite{knowledge_extract} go one step further, their goal is to directly extract the knowledge from flow charts without recognizing an explicit graph structure. Similarly, Wu~\etal~\cite{code_extract} want to generate code from given flow charts. Both works make strict assumptions about the given images and focus strictly on their use case.

In contrast, our approach aims at SVC more in general and does not demand a certain type of graph structure. Therefore, we strive to detect basic elements such as nodes and their content, as well as different types of edges and their weights. The final graph representation should be purely descriptive, without being specialized for any certain use case. Further, we alleviate the issue of little available, ground-truth annotated data \cite{scharfenberger2021augmented} by combining manually labeled with synthetic data.


% %% Todo
% To our knowledge, only one scientific paper so far deals with the topic of automatic graph recognition \cite{optical_graph_recognition}. This work only covers a part of our basic problem. It deals with the recognition of undirected graphs and their topology. A recognition of the topology is also one of the bases of our graph representation. The work tries to extract nodes as well as edges using methods of conventional computer vision and to build a graph representation. In the procedure the work describes a multi-step procedure with preprocessing, segmentation, topology recognition, and postprocessing. We use a very similar procedure for the recognition of graphs, only the preprocessing is omitted and an additional to the structure segmentation of the text is performed. The segmentation at our system is covered by different neural networks.
% Major differences are that these are graphs without text. The goal is a pure graph representation without their content. In addition, these are graphs that have been drawn uniformly by software.  

% opencv paper

% Optical Graph Recognition Christopher Auer, Christian Bachmaier, Franz J. Brandenburg, Andreas Gleißner, and Josef Reislhuber

% Erste Frage in wiefern unterscheidet sich deren Problem von unserem: 

% Deren Grundaufgabe: "In this paper, we proposeoptical graph recognition(OGR)asamethodtoau-tomatically extract the topological structure of a graph from its drawing"

% 1. undirected graphs G=(V,E)

% 2. Ussage of morphological image processing

% Anderer Benchmark (eventuell auch mit unserem vergleichen)

%3. preprocessing, segmentation, topologyrecognition, and postprocessing als 4 Phasen Prinzip

% Vergleich dazu bei uns: 
% Preprocessing entfällt,
% Segmentation macht bei uns Final ein Neuronales Netz in ihrem Fall openCV
% topologyrecognition machen wir beide 


% Sachen welche ähnlich oder gleich sind :

% 

% Wichtig hierbei war nur die Erkennung des Graphen wichtig nicht die Erkennung von Text



==> IEEEconf_ICPR2020/sections/3_dataset.tex <==
% \section{Dataset}

% Das Ziel war es einen Datensatz zu erstellen, der kann...
% keine implementierungs details

% \begin{itemize}
%     \item Eigenschaften Grafik - types, variations
%     \begin{itemize} % types
%         \item image size
%         \item random positioning
%         \item nodes (rectangle, ellipse) can but don't have to have edges
%         \item groupings (rectangle) - maybe 1 (no text)
%         \item edges (straight, striped) (tips: filled, lines) (uni-directional, bi-directional, no none) (max 1 right corner)
%         \item text (random, in nodes, numbers on edges (possible white background))
%         \item text size, line width
%         \item variation in drawing strategy %(cv2.LINE_4, cv2.LINE_AA, cv2.LINE_8)
%     \end{itemize}
%     \item ground truth
%     \begin{itemize}
%         \item BBs (mit Klassen..)
%         \item GraphRepräsentation
%     \end{itemize}
% \end{itemize}


% Statistiken, was ist im Ergebnis drin....

% Beispiele





\section{Synthetic Structured Visual Content}
% our main contribution... 

%\subsection{Goal}
The creation of SVCs in this work is subject to various targets. We generate images of different sizes that present nodes and edges connecting them. Furthermore, groupings of nodes are possible and random text fields are included in these images. In addition, different design choices are applied to these objects, to increase the possible variations.

A node can be a rectangle or an ellipse and displays text. Multiple nodes can be framed by a rectangular grouping. Each node can be connected to one or multiple other nodes or to a grouping by an edge, but it does not have to. A grouping itself can only be connected to other nodes outside, but not to nodes within itself. An edge can be a straight line or an angled one, while being uni-directional or bi-directional. A variation of these edges is striped and the arrow tips can be filled or just line-work. Each edge has a numerical weight, presented by a text near the line, sometimes with an additional white background, which could overlap with the edge itself. All variations mentioned are distributed uniformly. Furthermore, different text sizes are used in these images, as well as different line widths and drawing strategies such as anti-aliasing.

In our implementation, we used a grid structure to place the objects. At a random position within each cell there may either be a node, a background text or nothing. Textual content is chosen from a list \cite{text_source}. Then a number of edges is placed between the nodes, but no connection is made twice, also avoiding collisions with nodes. Edge weights between 0 and 1 are annotated as well. Just as the variations in design, all positional decisions are afflicted by randomness. The size of the image, grid structure and nodes are all chosen randomly, as well as the number of nodes, edges and other elements. An example of such an SVC can be seen in Fig. \ref{fig:example_synthetic_vs_disknet}a.

Together with these images, we generate ground truth data for all tasks. 
For the object detection, bounding boxes are stored for the objects and separately for text segments.
Nodes of all variations and groupings are labeled ``node'', while edges are differentiated by their start and end point within a bounding box. In our case these can be in two opposing corners (diagonal edges) or at two opposing side centers (horizontal and vertical edges). 
This leads to 8 different edge types as seen in Fig. \ref{fig:edges}. 
To also represent bidirectional edges, which have two end points, we add further 4 classes in the same way.
Since we encountered problems with very small bounding boxes and under represented classes, we chose to label diagonal edges, that fall into +/-2.5 degrees of 0/90/180/270 degrees with the closest horizontal or vertical label.
We save bounding boxes for all texts within a node, besides an edge or in the background according to their purpose: ``node", ``edge", or ``plain".

For graph recognition tasks, we directly create a document that describes the generated graph structure. In this document, there is a list of all nodes, specifying their id, content and potential sub nodes. If a node has a sub node it is considered a grouping. Likewise, a list of all edges is defined with an id, weight, source-node and target-node id and information regarding the arrow tips for each edge. 
%We add two uni-directional edges for each bi-directional edge.  

% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.5\linewidth]{IEEEconf_ICPR2020/figures/EdgeOrientation.pdf}
%     \caption{Classification of edge directions}
%     \label{fig:edge_orientation}
% \end{figure}

\setlength{\abovecaptionskip}{-6pt}
\setlength{\belowcaptionskip}{-30pt}
\begin{figure}[]
    \centering
    \includegraphics[width=0.9\linewidth]{IEEEconf_ICPR2020/figures/EdgeInformationNew.pdf}
    \caption{Statistics on Edge Classes}
    \label{fig:edges}
\end{figure}


%\subsection{Statistics}
In total, we generated 12,000 images and ground truths, with a 70\%, 20\%, 10\% split into train, validation, and test data.

These images contain a total amount of 167,685 objects, 94,701 of them are nodes and 72,984 are edges. A detailed description of the edges and their respective classes is shown in Fig. \ref{fig:edges}. 
Diagonal edges are much more likely than horizontal or vertical edges. Furthermore, in our implementation, an edge has a 20\% chance to be bi-directional. This is visible in the statistics, as for example \#bl2tr + \#tr2bl $\approx$ 4 * \#bi\_tl2br. 
The naming of the edge classes represent their orientation within their bounding box. For example, ``tl2br" means ``top-left to bottom-right", likewise ``l2r" means ``left to right" referring to a horizontal edge pointing right (see Fig. \ref{fig:edges}).
Furthermore, a distinction is made between bi-directional and unidirectional edges. We display an exemplary synthetic image as well as a real-world image from the DISKNET dataset in Fig. \ref{fig:example_synthetic_vs_disknet}.

% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Distribution of the element - classes}
% \label{table_elementdist}
% \centering
%         \begin{tabular}{l||c|c|c}
%         \hline
%         \bfseries Structures   & \bfseries Absolute    & \bfseries Percent of Total    & \bfseries Percent of Edges \\
%         \hline\hline
%         All                 & 16619                 &                       &   \\
%         \hline
%         \hline
%         Nodes               & 9381                  & 0.564                 &   \\
%         \hline
%         \hline
%         Edges - all         & 7238                  & 0.436                 &  \\
%         \hline
%         edge\_tl2br        & 1248                  & 0.075                 & 0.172 \\
%         \hline
%         edge\_t2b          & 114                   & 0.007                 & 0.016 \\
%         \hline
%         edge\_tr2bl        & 1294                  & 0.078                 & 0.179 \\
%         \hline
%         edge\_r2l          & 254                   & 0.015                 & 0.035 \\
%         \hline
%         edge\_br2tl        & 1289                  & 0.078                 & 0.178 \\
%         \hline
%         edge\_b2t          & 110                   & 0.007                 & 0.015 \\
%         \hline
%         edge\_bl2tr        & 1271                  & 0.076                 & 0.176 \\
%         \hline
%         edge\_l2r          & 227                   & 0.014                 & 0.031 \\
%         \hline
%         edge\_bi\_tl2br    & 643                   & 0.039                 & 0.089 \\
%         \hline
%         edge\_bi\_t2b      & 58                    & 0.003                 & 0.008 \\
%         \hline
%         edge\_bi\_tr2bl    & 610                   & 0.037                 & 0.084 \\
%         \hline
%         edge\_bi\_r2l      & 120                   & 0.007                 & 0.017 \\
%         \hline
%         \end{tabular}
% \end{table}


==> IEEEconf_ICPR2020/sections/4_methodology.tex <==
\section{Methodology}
Our goal is to extract the information from an image presenting SVC.
Therefore, we address the problem of mapping from an image showing a graph structure to a set of nodes and edges and their relation. In the following, we name this resulting set of nodes and edges graph representation. Specifically, our task describes the function
$$
Image \rightarrow \{Node\} \cup \{Edge\}.
$$

Nodes in our case are defined by their unique id and their textual content. Optionally, a node can contain a set of sub-nodes to define aggregations of nodes called groupings. Similar to nodes, edges are also defined by their id and their weights. In addition, an edge has a source and a target node. 

%$$
 %   Node := \{ID, Content, \{NodeID\}\}
%$$

%$$
  %  Edge := \{ID, Content, Node , Node\}
%$$


% introduction and why two methods
% \subsection{Traditional Approach: Conventional Computer Vision}

% Conventional computer vision methods use mostly pixel-based operations to gain structural information. The main task here is to differentiate between text and graph structures in the image. Therefore, we experimented with different methods to extract coherent regions of certain size and shape. These methods depend largely on the given image and its quality. Different images follow different rules in their content and therefore need to be treated individually. Another challenge to solve are interrupted lines. Such problems need to be detected and reconstructed accordingly. 

% Due to these challenges and various problems, that are discussed in the Section \ref{sec:discussion}, we did not pursue this approach any further.

% % Standard Computer Vision Approach
% Computer Vision tries to make machines capable of getting a high level understanding of visual content. Standard/Traditional approaches use specifically defined rules on pixel operations to gain structural information. We used...

% Core problems: differentiate lines of edges and lines of nodes

% Overall problem: Images vary a lot in style. No rules are able to adapt to all

% \subsection{Proposed Approach: Supervised Learning}
% Topic: supervised Machine Learning
% recent achievements
% Needs labels: none given
% In comparison to the conventional approach we use methods of machine learning, in particular we use object detection to recognize structures. In our case these are nodes and edges.
% As can be seen in Figure \ref{fig:pipeline}, an OCR is used in parallel to extract the texts with their bounding boxes from the image. Afterwards, the two results are combined to create a graph representation with the corresponding text assignment.\\
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/Pipline.png}
%     \caption{Showing the full Pipeline Scheme to generate the Graph Representation.}
%     \label{fig:pipeline}
% \end{figure}\\
% However, object detection is a supervised learning method, which means, we need labeled data to train a model. Since we do not have such data, we try to generate synthetic images with corresponding annotations.
% To achieve the best performances on real data, this synthetic data must be as realistic as possible.

%However, in order to perform object-detection, this must first be trained. This requires labeled data. Since no such dataset exists, we decided to generate synthetic data.

% \subsubsection{Synthetic Data Generation}

% problem no annotations -> supervised learning
% solution: create data with annotations
% show stats
% The goal is to generate images, that mimic a given set of real data while exhibiting high variation.  
% Since an infinite amount of variation is not feasible, we have decided on the following properties: Nodes exist as rectangles or ellipses. A node can contain text and/or other nodes. Edges always run between two nodes as a direct or angled line. They can also have arrowheads at both, one or none of its ends. The line can be solid or dashed, and the appearance of the arrowhead can vary. The weights of an edge rest on it or intersect the line. Also, for all elements, the size and line thickness can vary.\\

% moved to III dataset:
% In our implementation, nodes are distributed on a grid structure, varying in their position and shape. Their text content is selected from a list \cite{text_source}. Then a number of edges is placed between nodes, no connection is taken twice, and care is taken that an edge does not collide with a node, except for connections that run into a grouping. Along such an edge, the weight, a number between 0 and 1, is written to a random position.
% Additionally, background text is added.\\
% All of these actions are taken randomly, determined by a set of hyper-parameters.
% Therefore, we have generated a more difficult dataset than a real dataset, as it contains various anomalies. This is due to the generous use of random ranges, which sometimes creates more complexity than is needed later. 
% In total, we generated 12000 images, with a 70\%, 20\% and 10\% split into train, validation and test data. Additionally, we generated all bounding box annotations, text bounding boxes and ground truth graph representations for possible later evaluations. 



% If we could generate similar images with enough variety that mimic the given dataset, we could generate perfect ground truth annotations directly with them
% main parts: box nodes, round nodes, arrows + tips, straight and corner/bent, text within nodes, on edges and randomly within
% Variety: position, 

%%%%%%%%%%%%%%
% NEW 
%%%%%%%%%%%%%%

Given the generated dataset, containing images of SVC, bounding box annotations of all objects and ground truth graph representations, the problem can be seen as supervised learning formulation. Instead of defining all possible variations by hand as needed in the traditional approach, machine learning techniques are applied to generalize over a large set of variations provided by the dataset.

The task is divided into different steps (see Fig. \ref{fig:intro}). 
The first receives an image and is supposed to detect all structural components such as nodes and edges. This is done via common object detection methods, utilizing the generated bounding box annotations.
%
In parallel, text recognition methods are applied, which extract the textual content from the image together with a position.
%
The next step uses the detected objects and reconstructs their structural relation by means of nearest neighbour approaches and heuristics.
Here, the goal is to create a graph structure describing the connection between nodes by the different edges and the grouping relations.
%
After that, the extracted textual information are mapped to their matching nodes and edges and added to the final graph representation.

\subsubsection{Object Detection}
% The objects generated in our dataset are defined by a rectangular bounding box and a class label. Both nodes and groupings have the same class. Edges on the other hand are differentiated by their start and end points. Diagonal edges and angled edges go from one corner of their bounding box to another one (e.g. bottom-left to top-right). Horizontal and vertical edges go from the center of one side to the center of the opposite side of their bounding box (e.g. left to right). An edge is labeled horizontal or vertical if it is within +/- 2.5 degrees of being perfectly horizontal or vertical. Therefore, we have 4 diagonal classes, 2 horizontal and 2 vertical. Additionally, an edge could be bi-directional or non-directional, this leads to further 8 classes respectively. % because bi left to right == bi right to left 
We used a pretrained version of the YOLOv5 model \cite{yolov5} in its large configuration and fine tuned it on the training set of 8.400 images. We refrain from using flipping in the data augmentation step, as this would conflict with our definition of edge orientations. Furthermore, the Intersection over Union (IoU) threshold in training and detection should be set to zero, as overlapping bounding boxes are normal in this application. The result of this step are bounding boxes for each image, describing the position of nodes and different types of edges. However, we lose some information. By describing edges only via a bounding box and general direction, the exact course of an edge, is lost. While this may lead to problems when assigning the text to the edges it can be improved in the future.

% The model used for the object detection is YOLOv5 \cite{yolov5} with the large weight configuration. Important for our class labels is that in the data augmentation step, no flipping is involved. Furthermore, the IoU threshold in training and detection should be set to zero, as overlapping bounding boxes are normal in this application. % do we have to give specifications about the model here?? more in evaluation part
% explain different thoughts
\subsubsection{Text recognition}
% OCR and assignment to nodes and edges
% how did we assigne the textes to the nodes and the edges. 
% Problems of assign the text'bbs to edge bb's
Since text is an elementary component of graphs, it must also be included in the final graph representation. Because our object detection deals only with the detection of the structure, we used \textit{easy-OCR} \cite{EasyOCR} for the text. This text recognition works parallel to the object detection (see Fig. \ref{fig:intro}) and has no dependencies on it. It takes the same image as the object detection and returns a list of all detected texts, as well as their bounding boxes and positions. These are used later in the graph creation for the assignment.



% \subsubsection{Graph Creation}
\subsubsection{Create Graph Representation}
% bounding boxes to graph representation
% In this section the graph representation is the point of interest
% Assign the bb's of edges to the nodes
% Nodes and Groupings
The results from object detection and text recognition are now merged into a graph representation. This can be divided into two main steps:
\noindent \paragraph{Step 1} Construction of the graph structure\\
In this process, groupings are detected at the beginning. To do this, the overlaps of all bounding boxes are determined. If a box is almost completely inside another, it is considered a subnode with the larger node as the grouping.
Afterwards, the nodes are connected via edges. For this, the \textit{connection points} are searched for an edge on its bounding box.
The connection points represent the start and end points of an edge, which are derived by the edge direction class. For a diagonal or angled edge these points are in the corner of a bounding box, for a horizontal or vertical edge, they are on the center of a side.
For each connection point the next adjacent node is searched and connected to the edge. 
In the end, all elements are connected accordingly and we have created a graph structure, that contains all previously detected objects.
\noindent  \paragraph{Step 2} Text mapping:
After the graph structure has been created, the texts have to be assigned to the corresponding elements in the graph.
First, the overlap to the node boxes is determined for each text bounding box. If the overlap is large enough, the text is considered as a part of the node and added to it.
The remaining texts must therefore belong to edges, or have been placed freely in the image.
To assign the edges, all possible edge bounding boxes are determined for each text bounding box, based on their overlap.
Then the most probable edge bounding box for the text is determined, based on all possible courses of an edge within its bounding box. All remaining texts are assumed to be background texts and will not be added to the graph representation.








==> IEEEconf_ICPR2020/sections/5_evaluation.tex <==
\setlength{\abovecaptionskip}{-6pt}
\setlength{\belowcaptionskip}{-10pt}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\linewidth]{IEEEconf_ICPR2020/figures/fig4.pdf}
    \caption{Slightly wrong edge classifications do not hinder Graph Reconstruction}
    \label{fig:edges_detection}
\end{figure}

\setlength{\abovecaptionskip}{-0pt}
\setlength{\belowcaptionskip}{-0pt}
\begin{table}[b]
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{4pt}
\caption{\#Labels and $mAP@[.5, .95]$ in Percent. \\ The edge names  follow the naming scheme of \{StartingPoint\}2\{EndPoint\}, \textit{i.e.} ``tl2br" for ``top left to bottom right". The prefix ``Bi" indicates bidirectional edges.}
\label{tab:map}
\centering
        \begin{tabular}{c|cc|cc|cc|cc|c}
        \multicolumn{10}{c}{\uppercase{\textbf{Synthetic Testset}}}
        \\
        \hline
        &\textbf{tl2br} & \textbf{br2tl}   & \textbf{tr2bl} & \textbf{bl2tr}   & \textbf{r2l}  & \textbf{l2r}   & \textbf{t2b}  & \textbf{b2t}  &  \textbf{nodes} \\
        \hline
        \hline
        \#Labels & 1248  & 1289                                         & 1294  & 1271                      & 254    & 227  & 114    & 110    &  9381 \\
        \hline
       $mAP$ &  86.7  & 87.3                                         & 87.8  & 86.3                      & 48.6   & 48.9 & 37.6   & 47.6   &  99.5 \\
        \hline 
        \hline
        & \multicolumn{2}{c|}{\textbf{bi\_tl2br}}    & \multicolumn{2}{c|}{\textbf{bi\_tr2bl}}   & \multicolumn{2}{c|}{\textbf{bi\_r2l}} & \multicolumn{2}{c|}{\textbf{bi\_t2b}}  &  \textbf{all} \\
        \hline
        \hline
        \#Labels & \multicolumn{2}{c|}{643}               & \multicolumn{2}{c|}{610}& \multicolumn{2}{c|}{120} & \multicolumn{2}{c|}{58}  &   16619 \\
        \hline
        $mAP$ & \multicolumn{2}{c|}{79.9}               & \multicolumn{2}{c|}{77.9}& \multicolumn{2}{c|}{47.0} & \multicolumn{2}{c|}{43.6}  &   67.6 \\
        \hline
%         \end{tabular}
% \end{table}


% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{\#Labels and $mAP@[.5, .95]$ for DISKNET Test Set in Percent \\}
% \label{tab:map2}
% \centering
%         \begin{tabular}{cc|cc|cc|cc|c}

        \multicolumn{10}{c}{\uppercase{\textbf{DISKNET Testset}}}
        \\
        \hline
        & \textbf{tl2br} & \textbf{br2tl}   & \textbf{tr2bl} & \textbf{bl2tr}   & \textbf{r2l}  & \textbf{l2r}   & \textbf{t2b}  & \textbf{b2t}  &  \textbf{nodes} \\
        \hline
        \hline
        \#Labels & 55    & 21                                           & 15    & 63                        & 2      & 39  & 7     & 7     &  210  \\
        \hline
        $mAP$ & 39.9  & 54.4                                         & 71.9  & 46.4                      & 15.0   & 0.8 & 0.0   & 0.0   &  87.5 \\
        \hline 
        \hline
        & \multicolumn{2}{c|}{\textbf{bi\_tl2br}}    & \multicolumn{2}{c|}{\textbf{bi\_tr2bl}}   & \multicolumn{2}{c|}{\textbf{bi\_r2l}} & \multicolumn{2}{c|}{\textbf{bi\_t2b}}  &  \textbf{all} \\
        \hline
        \hline
        \#Labels & \multicolumn{2}{c|}{1}                 & \multicolumn{2}{c|}{0}  & \multicolumn{2}{c|}{0}   & \multicolumn{2}{c|}{9}    &   429 \\
        \hline
        $mAP$ &  \multicolumn{2}{c|}{0.0}               & \multicolumn{2}{c|}{N/A}& \multicolumn{2}{c|}{N/A} & \multicolumn{2}{c|}{5.8}  &   29.2 \\
        \hline
        \end{tabular}
\end{table}

\section{Evaluation}

\label{sec:eval}
In this section, we evaluate the performance of object detection, generated graph structure and the text recognition. 
% This section focuses first on the  datasets used for the evaluation, then on the applied metrics and finally on the most important numbers regarding the evaluation. We distinguish between the object detection, the graph structure and the OCR with the text assignment.

\subsection{Different Datasets}

To evaluate our pipeline we use four different datasets. We can divide these datasets into synthetic data and real data.

The synthetic dataset of 1,200 images is generated exactly as the training dataset and therefore has the same properties. 
From this dataset we take a subset of 30 clean, artefact-free images, as an adjusted version of the synthetic set.

For the real-world dataset, we manually annotated a subset from DISKNET~\cite{Disknet} containing 24 images. Again, we constructed an adjusted subset of 17 images, that do not include artifacts not available in our training set, such as curved edges.

%
\subsection{Metrics}

% Hier noch mehr lesefluss garantieren
We rely on established metrics to evaluate our results from the object detection. Whereas, to evaluate the graph structure and the text recognition and assignments, we define our own metrics, since this is a problem without easy computable well established metrics. We overcome the time complexity of other metrics by exploiting the positional information.

 

\subsubsection{Metrics for the Object Detection}

%%TODO Eventuell Jonas

To evaluate the object detection we use the $mAP$ defined as
$$
			    mAP = \frac{1}{|classes|}\sum_{c \in classes} \frac{\#TP(c)}{\#TP(c) + \#FP(c)},
$$

% mAP@.5:.95

\noindent where a true positive ($TP$) is a prediction bounding box A that has an $IoU(A,B)$ to a groundtruth bounding box $B$,
$$
			    IoU(A, B) = \frac{A \cap B}{A \cup B},
$$
greater than a threshold, otherwise it is a false positive ($FP$). Furthermore, we evaluate the $mAP$ averaged for $IoU$ thresholds from $0.5$ to $0.95$ with a step size of $0.05$ (COCO’s \cite{coco} standard metric, simply denoted as $mAP@[.5, .95])$.



\subsubsection{Metrics for the Graph Structure}
Evaluating graphs and their isomorphism is a complex problem. After the prediction the result contains a graph representation with nodes and edges. But it contains no information about which structure of the predicted graph is related to which structure in the ground truth graph representation. This metric is calculated via the IoU of the predicted bounding boxes and the ground truth boxes of the synthetic or real world data. We define 
$$
    IsomorphicError =  \#mNodes + \#mEdges,
$$
with $mNodes$ and $mEdges$ as the amount of nodes and edges in the prediction and the ground truth representation without a match. Therefore, this number combines false negatives and false positives. Similarly we also define the normalized
$$
\quad NormIsomorphicError = \frac{IsomorphicError}{\# Nodes + \# Edges}
$$ 
to be able to better compare graphs of different size. In addition, we also calculated this error measure only for the nodes as well as the edges. We take only the missing nodes and the missing edges for the isomorphic error and normalize them with the number of nodes or edges in the graph. Note the $NormIsomorphicError$ can be larger than 1 as there could be more nodes or edges predicted than existing in the image.

\subsubsection{Metrics for the Text Mapping and the Text Recognition}

To compare the results of our text recognition as well as our assignment of the texts within the pipeline we define another error measure. We use the Levenshtein Distance \cite{Levenshtein}. The Levenshtein Distance $L(X,Y)$ is defined as the minimum number of deletions, insertions and replacement operations to change text $X$ to text $Y$. With this we can define our 
$$  
TextRecError = \frac{  \sum_{S_{matched}}L(GT_{content}, P_{content}) }{ \sum_{S_{matched}}\#GT_{content}},
$$ with $S_{matched}$ as every matched structure, $GT_{content}$ as the content of the structure in ground truth, $P_{content}$ as the content of the structure in prediction and the amount of characters in the ground truth content $\#GT_{content}$.

\subsection{Results}
In the following sections we present the results, divided into the object detection part, the graph representation and the text recognition as well as their assignment.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{IEEEconf_ICPR2020/figures/realErrors.png}
    \caption{Example for human-created bad behavior (LEFT: merged edges; RIGHT: ambiguous weight positioning) graphs from the DISKNET dataset.}
    \label{fig:realErrors}
\end{figure}


\setlength{\abovecaptionskip}{-0pt}
\setlength{\belowcaptionskip}{-0pt}
\begin{table}[!b]
\renewcommand{\arraystretch}{1.3}
\caption{Normalized Isomorphic Error on the different Datasets. \\ Dir. $\widehat{=}$ if the graph is taken as a directed/undirected Graph.\\ BC. $\widehat{=}$   best Case $\quad $ WC. $\widehat{=}$  worst Case.}
\label{iso_error}
\centering
        \begin{tabular}{c||c||c|c|c|c|c}
        \hline
         & \bfseries Structure & \bfseries Dir. &  \bfseries Mean & \bfseries Std.& \bfseries BC. & \bfseries WC. \\ 
        \hline\hline
        %%%%%%%%%%%%
        % Synthetic Testset Table
        %%%%%%%%%%%%
        \multirow{5}{*}{\rotatebox[origin=c]{90}{\bfseries \makecell{Synthetic \\ Testset}}} & \multirow{2}{*}{Full Graph}
        %  \hline
         &\cmark  & 0.134  & 0.132 & 0 & 0.833\\
        & &\xmark  & 0.081  & 0.115 & 0 & 0.833\\
        % \cline{2-7}
        %  \hline
        \cline{2-7}
        & \multirow{1}{*}{Nodes}
                %  \hline
        & & 0.016  &  0.0479 & 0 & 0.5\\
        \cline{2-7}
            %  \hline
        & \multirow{2}{*}{Edges} & \cmark   & 0.287  & 0.281 & 0 & 3\\
             & & \xmark & 0.168  &  0.244 & 0 & 3\\
        \hline
        \hline
        %%%%%%%%%%%%
        % Adjusted Synthetic Testset Table
        %%%%%%%%%%%%
        \multirow{5}{*}{\rotatebox[origin=c]{90}{\bfseries \makecell{Adjusted \\ Synthetic \\ Testset}}} & \multirow{2}{*}{Full Graph}
        %  \hline
         &
         \cmark  
         &  0.043 & 0.057 & 0.0 & 0.2 \\
        & &\xmark & 0.03 & 0.053 & 0.0 & 0.2 \\
        % \cline{2-7}
        %  \hline
        \cline{2-7}
        & \multirow{1}{*}{Nodes}
                %  \hline
        & & 0.009 & 0.035 & 0.0 & 0.143\\
        \cline{2-7}
            %  \hline
        & \multirow{2}{*}{Edges} & \cmark   & 0.1 & 0.163 &  0.0 & 0.667\\
             & & \xmark & 0.068 & 0.152 & 0.0 & 0.667\\
        \hline
        \hline
        %%%%%%%%%%%%
        % Disknet Testset Table
        %%%%%%%%%%%%
        \multirow{5}{*}{\rotatebox[origin=c]{90}{\bfseries \makecell{Disknet \\ Testset}}} & \multirow{2}{*}{Full Graph}
        %  \hline
        %  \hline
         &\cmark  &  0.328 & 0.139 & 0.091 & 0.654 \\
         & &\xmark  & 0.297 & 0.122 & 0.091 & 0.556 \\
        \cline{2-7}
        & \multirow{1}{*}{Nodes} 
        &  & 0.037 & 0.076 & 0.0 & 0.273\\
        \cline{2-7}
              & \multirow{2}{*}{Edges} 
            %  \hline
            & \cmark    & 0.613 & 0.233 & 0.143 & 1.0\\
             & & \xmark & 0.553 & 0.211 & 0.143 & 1.0\\
        \hline
        \hline
        %%%%%%%%%%%%
        % Adjusted Disknet Testset Table
        %%%%%%%%%%%%
        \multirow{5}{*}{\rotatebox[origin=c]{90}{\bfseries \makecell{Adjusted \\ Disknet \\ Testset}}} & \multirow{2}{*}{Full Graph}
        %  \hline
         &\cmark  & 0.325  & 0.139 & 0.091 & 0.654\\
        & &\xmark  & 0.291  & 0.123 & 0.091 & 0.556\\
        % \cline{2-7}
        %  \hline
        \cline{2-7}
        & \multirow{1}{*}{Nodes}
                %  \hline
        & & 0.021  &  0.062 & 0.0 & 0.25\\
        \cline{2-7}
            %  \hline
        & \multirow{2}{*}{Edges} & \cmark   & 0.622  & 0.226 & 0.2 & 1.0\\
             & & \xmark & 0.558  &  0.213 & 0.2 & 1.0\\
        \hline
        \end{tabular}
\end{table}


\subsubsection{Evaluation of the Object Detection}
% old
% We evaluated object recognition on the synthetic test set and on the DISKNET test set, visible in  Table \ref{tab:map}. It should be noted that the DISKNET test set is small and in some cases does not contain any labels of a category. As seen in the table, horizontal and vertical edges pose a much harder problem for the object detection than the diagonal edges. Furthermore, after manual evaluation we noticed, that most errors do not come from missed detections but from wrong classifications, meaning an edge from right to left is detected as an edge from bottom right to top left. It can be argued that such an error is less bad than a complete miss.

% Data sets
We evaluated the object detection on the synthetic test set and the DISKNET test set, visible in Table \ref{tab:map}.
% Meaning of numbers
The nodes and the most common edge types are detected very well by the model, while the less common types are recognized not as good. The comparison to the real world data set however shows, that those edge types are also less common there or not even present at all. 
% Bad
As seen in the table, horizontal and vertical edges pose a much harder problem for the object detection than the diagonal edges. This can be due to their generally smaller bounding box.
% Good 
After manual evaluation we noticed, that most errors do not come from missed detections but from wrong classifications. This means that an edge from bottom to top is detected as an edge from bottom left to top right. It can be argued that such an error is less bad than a complete miss, since the graph reconstruction can still work correctly in those situations (see Fig. \ref{fig:edges_detection}).




% As we only have ground truth bounding box labels for the synthetic data we evaluate the object detection only on the synthetic test dataset as visible in table \ref{tab:map}.


% \begin{table}[H]
%     \centering
%   \begin{tabular}{ccc}
%     \hline
%               Class &    Labels &            mAP@.5:.95:  \\
%     \hline
%                  all   &     16619 &     0.676  \\
%                 node   &      9381 &   0.995  \\
%          arrow\_tl2br  &      1248 &            0.867  \\
%           arrow\_t2b  &       114 &         0.376  \\
%          arrow\_tr2bl  &      1294 &          0.878  \\
%           arrow\_r2l  &       254 &         0.486  \\
%          arrow\_br2tl  &      1289 &        0.873  \\
%           arrow\_b2t  &       110 &            0.476  \\
%          arrow\_bl2tr  &      1271 &          0.863  \\
%           arrow\_l2r  &       227 &           0.489  \\
%       arrow\_bi\_tl2br &       643 &            0.799  \\
%         arrow\_bi\_t2b &        58 &            0.436  \\
%       arrow\_bi\_tr2bl &       610 &             0.779  \\
%         arrow\_bi\_r2l &       120 &            0.47  \\
%     \hline
%     \vspace{0.1cm}
%     \end{tabular}
    
%     \caption{Showing the results of the object recognition on synthetic test set.}
%     \label{tab:table_object_rec}
% \end{table}




\subsubsection{Evaluation of Graph Representations}

% Table \ref{iso_error} shows the results of the normalized isomorphic error for a directed or undirected graph on the four different datasets. The model performed best on the adjusted synthetic dataset. The mean normalized isomorphic error of DISKNET testset does not differ a lot to the adjusted DISKNET testset.

% As visible the detection of the nodes works really well in all of the datasets. An example of this is shown in Table \ref{iso_error}, presenting the synthetic dataset. We were able to achieve that all nodes in some DISKNET pictures were recognized. 
% The detection of the edges is much more difficult in the real world dataset but not impossible. We observe some images where every edge is detected. Notice here, that every wrong mapping also results in a higher isomorphic error. Therefore, the isomorphic error on the edges on DISKNET testset of 0.613 is a result of the heuristic mapping and the edge detection. It is also visible that the edge direction seem to be a hard problem, as the mean of the isomorphic errors differs a lot with the direction of the edges in every dataset.

% Hier noch sagen das der Sprung von syntethischen zu Realen das Ganze nicht so stark verbessert und eine System herausgekommen ist, welches in der Lage ist solche Repräsentationen auch auf realen Bildern zu erstellen.

% Data sets
We evaluated the reconstructed graph representations on all four test sets, visible in Table \ref{iso_error}. The normalized isomorphic error is calculated in two versions, where the first one includes wrong directions of the edges in the error, while the second does not and only measures the undirected graph.
% Meaning of numbers
The nodes are again the easiest part and are recognised almost perfectly on average even in the real world dataset.
Edges however are more difficult, while the detection of their direction is a big part of their error.
% Bad
Furthermore, the mapping between edges of the ground truth and the detection results is very difficult.
In this implementation, we used heuristics to approximate a one to one mapping, which obviously can lead to problems.
This also means that one wrong assignment of an edge to a node can lead to two errors, as it counts towards a missing edge on the correct node and a false edge on that node.
% Good 
Nevertheless, in multiple cases the graph reconstruction was perfect and able to create the wanted graph representation.



% \begin{table}[H]
%     \begin{center}
%         \begin{tabular}{ccc}
%         \hline
%         %  \hline
%         dataset & Mean & Std. \\
%         \hline
%         Synthetic Test Set & 0.134  & 0.132 \\
%         Adjusted Synthetic Test Set & 0.043 & 0.057 \\
%         Disknet Test Set &  0.328 & 0.139 \\
%         Adjusted Disknet Test Set &  0.325 & 0.139\\
%         \hline
%     \end{tabular}
%     \end{center}

%     \vspace{0.1cm}
%     \caption{Showing the Isomorphic Error results on the different dataset.}
%     \label{tb:graph_res}
% \end{table}

 



% \begin{table}[H]
%     \begin{center}
%         \begin{tabular}{ccc}
%         \hline
%         %  \hline
%         Structure & Mean & Std. \\
%         \hline
%         Nodes & 0.016 & 0.0479 \\
%         Edges & 0.287 & 0.281 \\
%         \hline
        
%     \end{tabular}
%     \end{center}

%     \vspace{0.1cm}
%     \caption{Isomorphic Error Edges and Nodes on the Testset normalized.}
%     \label{tb:graph_res_edges_nodes}
% \end{table}






\subsubsection{Evaluation of Text Mapping and the Text-Recognition}
% In the evaluation of text recognition and text assignment (see Table \ref{ocr_error}), we observe the worst result in the synthetic testset. The best text-recognition error we observe in the adjusted DISKNET testset.
% If we look at the error on the synthetic testset we can see that the worst case error on the synthetic testset seems very high. This is caused by pictures with only few nodes, caused by the probabilistic generation, that are highly influenced if one node is not detected and miss leading mappings take place. 

% Data sets
We evaluated the text recognition and text assignment on all four test sets, visible in Table \ref{ocr_error}. 
% Meaning of numbers
We observe, that the text recognition is on average better in the real world data set than in the synthetic data set.
% Bad
Notice, that the error could be high, when a node is not detected, and therefore its text is falsely mapped. This influence is higher if there are only few nodes in the image.
% Good 
The text recognition however is not the main task of our work and it is modular and easy exchangeable.

% \begin{table}[H]
%     \begin{center}
%       \begin{tabular}{ccc}%{m{1cm}m{1cm}m{1.5cm}}
       
%             \hline
            
%             dataset & Mean & Std. \\
%             \hline
%             Synthetic testset & 0.423 & 0.429 \\
%             Adjusted Synthetic testset & 0.29 & 0.115 \\
%             Disknet testset & 0.254 & 0.214 \\
%             Adjusted Disknet testset & 0.20 & 0.187 \\
%             \hline
%         \end{tabular}  
%     \end{center}
    
%     \vspace{0.1cm}
%     \caption{Showing the OCR Error results on the different dataset.}
%     \label{tb:ocr_res}
% \end{table}


\section{Discussion}
\label{sec:discussion}

% old school computervision

% KLären warum OCR in Testset so hoch ist

% pro, cons and limitations

% \begin{figure*}[t]\label{gen_img}
% \centering
% \begin{tabular}{cc}
%     \includegraphics[width=0.45\linewidth,height=0.3\linewidth]{IEEEconf_ICPR2020/figures/generated_arrowsMerge.jpg}
%     &
%     \includegraphics[width=0.45\linewidth,height=0.3\linewidth]{IEEEconf_ICPR2020/figures/disknet_arrowsMerge.png}  \\
%     \footnotesize{(a) Example of our generated dataset.} & 
%     \footnotesize{(b) Example from the DISKNET dataset.}
% \end{tabular}
% \caption{Overlapping arrows can be interpreted as a merge.}
% \label{fig:mergeArrows}
% \end{figure*}

% \begin{figure*}[t]\label{gen_img}
% \centering
% \begin{tabular}{cc}
%     \includegraphics[width=0.45\linewidth,height=0.3\linewidth]{IEEEconf_ICPR2020/figures/generated_weights.jpg}
%     &
%     \includegraphics[width=0.45\linewidth,height=0.3\linewidth]{IEEEconf_ICPR2020/figures/disknet_weights.PNG}  \\
%     \footnotesize{(a) Example of our generated dataset.} & 
%     \footnotesize{(b) Example from the DISKNET dataset.}
% \end{tabular}
% \caption{Ambiguous positioning of edge weights exist in both synthetic and real data sets}
% \label{fig:weightPositioning}
% \end{figure*}


% \begin{figure*}[t]\label{gen_img}
% \centering
% \begin{tabular}{cc}
%     \includegraphics[width=0.45\linewidth,height=0.3\linewidth]{IEEEconf_ICPR2020/figures/10815.jpg}
%     &
%     \includegraphics[width=0.45\linewidth,height=0.3\linewidth]{IEEEconf_ICPR2020/figures/10815_reconst.jpg}  \\
%     \footnotesize{(a) Example of our generated dataset.} & 
%     \footnotesize{(b) Graphical reconstruction of the detected structure of the graph.}
% \end{tabular}
% \caption{A synthetic graph with a graphical representation of the recognized structure. Thereby graphical details, like the shape of a node, are no longer considered. The respective elements are drawn with their corresponding ID. It can be seen that the edge from node 2 to 5 is lost in the recognition. Consequently, the \textit{IsomorphicError} is 1 and the \textit{NormIsomorphicError} $1/14$.}
% \label{fig:reconstruction}
% \end{figure*}

\begin{table}[t]
\renewcommand{\arraystretch}{1.3}
\caption{Text Recognition Error \\ BC. $\widehat{=}$  best Case $\quad $ WC. $\widehat{=}$  worst Case.}
\label{ocr_error}
\centering
        \begin{tabular}{c||c|c|c|c}
        \hline
        \bfseries Dataset & \bfseries Mean& \bfseries Std. &\bfseries BC. & \bfseries WC. \\
        \hline\hline
        Synthetic Testset & 0.423 & 0.429 & 0.0 & 13.0 \\
        Adjusted Synthetic Testset & 0.29 & 0.115 & 0.091 & 0.474 \\
        Disknet Testset & 0.254 & 0.214 & 0.039 & 0.692 \\
        Adjusted Disknet Testset & 0.2 & 0.187 & 0.039 & 0.692 \\

        \hline
        \end{tabular}
\end{table}


Comparing the results of our evaluation is very difficult because there are no comparable works on this task. Existing works address problems such as recognising structures and assigning it to different classes, as \cite{scharfenberger2021augmented}, because of the different task they are not suitable for comparison.
The evaluation shows that nodes themselves can be detected very confidently, while edges pose some problems. In general, horizontal or vertical edges are harder than diagonal edges, which can be due to their smaller bounding box size, the fact that they are less common in the dataset or due to the observation, that they are not always missed but incorrectly classified. It can be argued, that an edge from left to right which is detected as an edge from bottom left to top right is less bad than a complete miss.

Another problem with the detection of edges is their direction (c.f. Table \ref{iso_error}). Apparently the arrow heads are too small to be confidently detected.
In the generation, some problems producing ambiguous graphs are not excluded, since they also represent existing challenges. In Fig. \ref{fig:realErrors} two examples of such real world difficulties are shown. %The same problems arise in the generation, since overlapping edges are not excluded. 
Furthermore, we show that a model is capable of generalizing over a large dataset, can extract the core structures of SVCs and apply them, also to maybe less complex SVCs. Therefore it is no problem, if the training data is sometimes a bit harder than the later real world use case. We show further examples in the supplementary material.

% in some situations the randomly generated dataset comes with problems that are more difficult than the real world data, but it is shown that a model that is able to learn those hard problems can also manage the easier versions. Therefore, the dataset can include more difficulties than needed in the end to conquer the real world challenge.


% The following sections discuss the different shortcomings and possible improvements of our approach.


% future work
% \subsection{Traditional Approach: Computer Vision}
% This method is highly dependent on the given image and needs to be adjusted accordingly. Therefore, good results are only achievable with heavy fine-tuning. Since our task involved real world images with lots of variation, this approach is not feasible. The data varies too much to create a fixed set of rules that applies on all images. 

% \subsection{Proposed Approach: Synthetic to Real}
In our synthetic to real approach we can divide the limitations into two categories. One deals with the influence of the synthetic dataset. The second focuses on the applied method. 

\label{sec:limitations}
\subsubsection{Dataset}
The synthetic dataset provides first good approaches to generate different graphs. However, there are many variations that can be added to this dataset. For example, round edges and further edge types are possible, together with additional class labels representing their directions. Also, multiple nested groupings are missing and more shapes of nodes would be a useful extension. The horizontal as well as the vertical edges seem to be underrepresented in the dataset, which leads to a worse recognition results of these. 

Furthermore, the dataset does not contain any additional information, such as legends. These would be an interesting special case, since they often show elements of the graph without having a semantic meaning for the graph itself.
%
In general, our synthetic set is randomly generated. Therefore, the layouts and structures are also random in contrast to diagrams created by humans. This results in the entire diagram being distributed much more evenly in the image than it is often the case in reality. In reality, you often find converging structures that have many edges running up to each other. Such structures are underrepresented in the training set.
%
For further improvements, it would be interesting to extend the synthetic dataset to be able to represent even more real world graphs.


\subsubsection{Methods}
One of our main methodological limitation is the heuristic assignment of text to edges. This constraint originates in the problem, that we only work with bounding boxes of edges and lost the information about their exact path. Additionally, real world images do not follow any rule on how to assign weights to edges and therefore it is difficult to design a general heuristic. Similarly, our nodes are detected and processed only by their bounding boxes too. Even though this did not lead to any problems now, it maybe would be better to switch from an object detection via bounding boxes to segmentation masks, especially for better edge detection.


% % 

% \section{Object Detection}

% \begin{tabular}{ccccc}
%     \hline
%               Class &    Labels &        P &       R &    mAP@.5:.95:  \\
%     \hline
%                  all   &     16619 &    0.866 &   0.685 &   0.676  \\
%                 node   &      9381 &    0.996 &   0.997 &   0.995  \\
%          arrow\_tl2br  &      1248 &    0.895 &   0.889 &   0.867  \\
%           arrow\_t2b  &       114 &    0.817 &   0.386 &   0.376  \\
%          arrow\_tr2bl  &      1294 &    0.915 &   0.878 &   0.878  \\
%           arrow\_r2l  &       254 &    0.839 &   0.533 &   0.486  \\
%          arrow\_br2tl  &      1289 &    0.915 &   0.879 &   0.873  \\
%           arrow\_b2t  &       110 &    0.908 &   0.509 &   0.476  \\
%          arrow\_bl2tr  &      1271 &    0.897 &    0.87 &   0.863  \\
%           arrow\_l2r  &       227 &    0.813 &   0.538 &   0.489  \\
%       arrow\_bi\_tl2br &       643 &    0.803 &   0.782 &   0.799  \\
%         arrow\_bi\_t2b &        58 &    0.813 &   0.379 &   0.436  \\
%       arrow\_bi\_tr2bl &       610 &    0.785 &   0.762 &   0.779  \\
%         arrow\_bi\_r2l &       120 &    0.859 &   0.507 &   0.47  \\
%     \hline
% \end{tabular}
%%% Test


% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Normalized Isomorphic Error on Adjusted Synthetic Testset}
% \label{iso_error_adjusted_synthetic}
% \centering
%         \begin{tabular}{c||c|c|c|c|c}
%         \hline
%         \bfseries Structure & \bfseries Dir. & \bfseries Mean & \bfseries Std. & \bfseries BC. & \bfseries WC. &  
%         \hline\hline
%         Full Graph &\cmark  &  0.043 & 0.057 & 0.0 & 0.2 \\
%          &\xmark & 0.03 & 0.053 & 0.0 & 0.2 \\
%         \hline
%         %  \hline
%         \hline
%         Nodes & & 0.009 & 0.035 & 0.0 & 0.143\\
%         \hline
%         \hline
%               Edges  
%             %  \hline
%             & \cmark   & 0.1 & 0.163 &  0.0 & 0.667\\
%              & \xmark & 0.068 & 0.152 & 0.0 & 0.667\\
%         \hline
%         \end{tabular}
% \end{table}
    
% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Normalized Isomorphic Error on Disknet Testset}
% \label{iso_error_disknet}
% \centering
%         \begin{tabular}{c||c|c|c|c|c}
%         \hline
%          \bfseries Structure & \bfseries Dir. & \bfseries Mean &\bfseries Std.  & \bfseries BC. & \bfseries WC. &  
%         \hline\hline
%         Full Graph 
%         %  \hline
%          &\cmark  &  0.328 & 0.139 & 0.091 & 0.654 \\
%          &\xmark  & 0.297 & 0.122 & 0.091 & 0.556 \\
%         \hline
%         %  \hline
%         \hline
%         Nodes 
%         &  & 0.037 & 0.076 & 0.0 & 0.273\\
%         \hline
%         \hline
%               Edges 
%             %  \hline
%             & \cmark    & 0.613 & 0.233 & 0.143 & 1.0\\
%              & \xmark & 0.553 & 0.211 & 0.143 & 1.0\\
%         \hline
%         \end{tabular}
% \end{table}

% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Normalized Isomorphic Error on Adjusted Disknet Testset}
% \label{iso_error_adjusted_disknet}
% \centering
%         \begin{tabular}{c||c|c|c|c|c}
%         \hline
%          \bfseries Structure & \bfseries Dir. & \bfseries Mean & \bfseries Std. & \bfseries BC. & \bfseries WC. &  
%         \hline\hline
%         Full Graph
%          &\cmark  &  0.325 & 0.139 & 0.091 & 0.654\\
%          &\xmark  & 0.291 & 0.123 & 0.091 & 0.556\\
%         \hline
%         %  \hline
%         \hline
%         Nodes && 
%          0.021 & 0.062 & 0.0 & 0.25\\
%         \hline
%         \hline
%               Edges 
%             %  \hline
%             & \cmark   & 0.622 & 0.226 & 0.2 & 1.0\\
%              & \xmark & 0.558 & 0.213 & 0.2 & 1.0\\
%         \hline
%         \end{tabular}
% \end{table}






==> IEEEconf_ICPR2020/sections/6_conclusion.tex <==
\section{Conclusion}
By storing the graph representation of SVC, the contained information within the image can be more easily accessed and utilized by other processes.
The automated parsing of such graph structures from SVC, however, is a challenging problem. To approach this, we have generated a synthetic automatically generated dataset which shares structures with its real counterpart. Through the automated dataset generation we gather annotations required for the training of deep learning models and enable tasks such as the parsing of graph structures. For the latter, our method matches detected nodes and edges with their respective captions based on spatial coordinates. 

We show promising results not only on the synthetic data but also on real world examples. Furthermore, we delineate potential limitations of our approach and, thereby, demonstrate the feasibility of our approach (\textit{i.e.} generating synthetic data, training on the aforementioned, applying the model on real world data) for SVC. Our approach allows for easily scalable training of performant models with only little manual annotation effort for, \textit{e.g.}, real world data. The \href{{https://bit.ly/3jN1pJJ}}{dataset} is publicly available. 
 We expect that our work will further enable easier automated analysis of SVC.



==> IEEEconf_ICPR2020/sections/TODO.tex <==
Pfeile Begrifflichkeiten klären START und ENd Taget und source etc

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> rebuttal/rebuttal.tex <==


% \documentclass[10pt,twocolumn]{article}
% \begin{document}




\section{Rebuttal}
We would like to thank all the reviewers for their thoughts and valuable feedback on our work of automatically recovering graph structures from SVC. We incorporate these into the revised version of our work.
We are glad that the reviewers agree on the relevance of our proposed dataset, which enables machine learning techniques to conquer the problem of automatic analysis of SVC. As a result to the comments of Reviewers \#3 and \#5 we decided to make the dataset available at \href{https://bit.ly/3jN1pJJ}{https://bit.ly/3jN1pJJ} prior to publication. We also show additional results in the supplementary. We further address some common concerns of the reviewers below:

\textcolor{red}{\textbf{Reviewer \#3}}:
\textbf{``A simplification of the adopted metrics should be considered [\dots]"}:
We understand that as the metrics are not widespread they are more difficult to interpret. However, applying a simplified variant to display errors graph reconstruction seems difficult. While one could consider the cardinality of missing node/edge sets this metric would struggle with not being normalised and thus has very little meaningfulness. We display the normalised values in our evaluation scheme for the individual detection of nodes and edges also in Table 2.

\textcolor{red}{\textbf{Reviewer \#4}}:
% \textbf{How does angled edges been recognized in our representation and in the dataset?}
\textbf{On the representation of angled edges}:
% We have chosen the corners of the bounding box of an angled edge as the start and end point of the arrow. For an example, we have thus classified an angled edge that starts in the upper left corner and goes across the upper right corner to the lower right corner as tl2br and resprectiv to this as an diagonal edge. Therefore, our goal was to identify every type of edges in a uniform way as a whole and not as two edges. 
% Alternative: 
We define edge types by their start and end point within their bounding box.  Therefore, an angled edge with a corner and a diagonal edge have the same class label, if they both start and end in the same corners. The exact path, whether its straight for a diagonal edge or angled for an edge with one corner, is irrelevant in this implementation.
Even future work with rounded edges could be implemented in this way.
Our reasoning behind this decision was that for the graph reconstruction we are typically not interested in the type of path an edge takes as their drawings can become quite convoluted, and, thus, only focus on the general connection between nodes.

As such the angled edges are not overlooked, but they face similar problems as not angled edges with the detection of the directions (specifically the detection of arrow tips). The direction of the edge is a difficult task, as the only difference between \textit{i.e.} a bidirectional arrow and an unidirectional one is the head of the arrow. This is a common reason for errors on the synthetic and on the real-world dataset. We have clarified these concerns in the main paper.

\noindent\textbf{``Table 1 is a little confusing, because of mixing \#labels and mAP without explicitly labelling the rows in the table."}:
We acknowledge this and we have clarified Table 1 in the revised version. 
Furthermore, we appreciate Reviewer \#4's stance on our evaluation. Since there are, to the best of our knowledge, no results that address exactly the recognition of structure and the building of representations within flow charts, straight comparisons were not possible. On a related note, we see this as additional aspect of our work to shed light on this problem to enable comparison and mutual improvement for the analysis of SVC.


\textcolor{red}{\textbf{Reviewer \#5}}:
\textbf{``The idea to generate synthetic data for such kind of
problem is not new [\dots]"}:
While the use of synthetic data has been increasing recently for various vision domains including document analysis, there currently exists no work which allows for the concrete analysis of structured visual content the same way as our SSVC.
Even though the core idea of our dataset generation approach can be easily extended in many ways, we show
% The main contribution lies in the presented set of minimal requirements a dataset for this task has to have and we show that 
this iteration of our dataset already enables machine learning models to handle several problems of SVC well. This does not only include the SVC images themselves, but also all the ground truth information for the object detection and the graph representation.

The size of the generated dataset is not limited in any way and the richness of content in the SVCs can be extended and adapted to the desired needs. 
% While we publish this dataset, it should be noted that this is not a final and perfect dataset. 
We note, that this is a base that can be used for comparison and future work can construct larger more complex versions following our proposed pattern.

\noindent\textbf{``[\dots]~the dataset suffers from unrealistic representations."}:
It has to be said that the data set certainly contains representations that are not realistic in terms of a perfect and beautiful flow chart. But most of them are comparable to examples in the DISKNET dataset. Here, many of the graphs created by humans are not unambiguous and present the same "unrealistic" representations. Similarly, the appearance of text seems to be sometimes better and sometimes worse, especially in relation to the placement of legends. 
Our experiments showed that a machine learning model trained on our dataset is able to learn the core concepts and can handle more difficult data in the training than it may see in the real application later. Therefore, it is no problem to include difficult and rarely unrealistic representations if the core concept is similar enough to the desired application.
% The aim here was to make the representations more difficult to learn a more difficult problem rather than an easier problem, as this would simply allow the recogniser to learn more difficult cases.


\noindent\textbf{Changes in the related work section and strengthening of the links to other works}:
We have expanded our related work in the revised version, including other graph structure generating methodologies from the field of mathematical form recognition as well as the other recommended literature. Especially the two papers on edit distance and subgraph detection show the possibilities of establishing such metrics and the difficulty of the problem. Work on table recognition or element localization is useful as a preliminary step to our work, in which the SVC must first be extracted from the document.
% Additionally, the localisation of elements within the flow chart is an important part of the pipeline. 
However, albeit several of these works being related they neither provide direct solutions to the problems of our task nor are easily transferable to it. As such we see not only our dataset but also our proposed graph extraction process from SVC as a novel contribution.




% \textbf{on the interpretability of our work}:
% % - establishing stronger links to other works,
% % - showing more examples of the dataset and the results
% % - commenting on the evaluation metrics in more detail
% % explain with reference to other paragraphs

% We understand that it is difficult to interpret the results without any comparisons to other works, but sadly there are none yet.

% This is another reason why this idea has to be published, so that it enables comparison and mutual improvement.
% We realise that in our attempt to give a very neutral and truthful presentation of the achieved results, we focused much more on the problems we want to fix, than presenting the actual goal that we achieved. The approach works very well for most graphs and often only fails at the same things a human fails when he is faced with the same SVC. It has a near 100\% detection rate of nodes and the edge detection is good enough so that the graph reconstruction works correctly in most cases. The most difficult task for now is the assignment of weights to their edges as this is often very ambiguous. In addition, the metrics are not perfect either. For example, if an edge from A to B is recognized as an edge from A to C, then it is counted as two errors since it is missing at B and wrongly added to C. Here, the main problem is to match detected edges with edges in the ground truth, but this is a very hard problem and out of the scope of this first approach.
% We tried to include those remarks and positive comments about the achieved goal now in this work and hope that future work introduces better metrics, that show the performance more clearly. We also included more positive examples in the supplementary.
% - Tabelle 1 ist mir absicht so aufgebaut (#Labels über mAP), damit zu erkennen ist, wie stark sich ein Fehler auswirkt (je weniger Labels, desto sträker der Einfluss) (R4)

\\
\vspace{5pt}
\noindent We thank the reviewers again for their time and truly
hope that our rebuttal will be considered in the discussions
before reaching a final decision.

% \clearpage



%synthetic dataset is not yet publicly available

%A simplification of the adopted metrics should be considered: it is hard to understand if the method works well or not because of a very huge set of numbers

% more examples of the generated dataset should be presented to the reader
% --> google drive
% --> supplementary

% the lack of explanation for angled edges, which are briefly mentioned, but all edge classes only represent one direction

% Table 1 is a little confusing, because of mixing #labels and mAP without explicitly labelling the rows in the table

% no comparison to other works, but if none of them are producing the same output representation, it is understandable that there cannot be any direct comparison
% --> eval comparison not possible

% The SOTA review is very short and are some missing
% reference. Ref [5][6] are not representative of the SOTA. I
% suggest for example the following:
% 1- T. N. Le, M. M. Luqman, A. Dutta, P. Heroux, C. Rigaud,
% C. Guerin, P. Foggia, J. Burie, J. Ogier, J. Llados, and S.
% Adam, � Ssgci: subgraph spotting in graph representations
% of comic book images, � Pattern recognition letters, 2018.

% 2- Z. Abu-Aisheh, B. Ga�zere, S. Bougleux, J. Ramel, L.
% Brun, R. Raveaux, P. H�roux, and S. Adam, � Graph edit
% distance contest 2016: results and future challenges, �
% Pattern recognition letters, vol. 100, p. 96�103, 2017. 

% 3- Have a look at the IAPR TC10 datasets page :
% https://iapr-tc10.univ-lr.fr/?page_id=71

%Some references to Mathematical expressions recognition (R5)

%The promise to make the dataset publicly available is not
%achieved yet.

% %dataset suffers from unrealistic representations. For
%  example textual placement is more randomly distributed in
% general than that of the dataset

% We get the impression of a
% non achieved goal if thinking at a general purpose
% representative dataset

% Disagree against no contribution

% \end{document}






==> sections/TODO.tex <==
Pfeile Begrifflichkeiten klären START und ENd Taget und source etc
